Quantum Approximate Optimisation Applied to Graph Similarity

Quantum computing promises solutions to classically difficult and new-found problems through controlling the subtleties of quantum computing. The Quantum Approximate Optimisation Algorithm (QAOA) is a recently proposed quantum algorithm designed to tackle difficult combinatorial optimisation problems utilising both quantum and classical computation. The hybrid nature, generality and typically low gate-depth make it a strong candidate for near-term implementation in quantum computing. Finding the practical limits of the algorithm is currently an open problem. Until now, no tools to facilitate the design and validation of probabilistic quantum optimisation algorithms such as the QAOA on a non-trivial scale exist. Graph similarity is a long standing classically difficult problem withstanding decades of research from academia and industry. Determining the maximal edge overlap between all possible node label permutations is an NP-Complete task and provides an apt measure of graph similarity. We introduce a novel quantum optimisation simulation package facilitating investigation of all constituent components of the QAOA from desktop to cluster scale using graph similarity as an example. Our simulation provides flexibility and performance. We investigate eight classical optimisation methods each at six levels of decomposition. Moreover an encoding for permutation based problems such as graph similarity through edge overlap to the QAOA allows for significant quantum memory savings at the cost of additional operations. This compromise extends into the classical portion of the algorithm as the inclusion of infeasible solutions creates a challenging cost-function landscape. We present performance analysis of our simulation and of the QAOA setting a precedent for investigating and validating numerous other difficult problems to the QAOA as we move towards realising practical quantum computation.

==> proposal.tex <==
\newcommand{\namelistlabel}[1]{\mbox{#1}\hfil}
\newenvironment{namelist}[1]{%1
\begin{list}{}
    {
        \let\makelabel\namelistlabel
        \settowidth{\labelwidth}{#1}
        \setlength{\leftmargin}{1.1\labelwidth}
    }
  }{%1
\end{list}}
\begin{document}
\begin{namelist}{xxxxxxxxxxxx}
\item[{\bf Title:}]
	Quantum Graph Similarity and Applications
\item[{\bf Author:}]
	Nicholas Pritchard
\item[{\bf Supervisor:}]
	Professor Jingbo Wang and Professor Amitava Datta
\item[{\bf Degree:}]
	BSc(Hons.)
\end{namelist}
\section*{Background}
The goal of quantum computing is the exploit the complexity of quantum systems for useful computation. Such a motivation arises from the fact that despite decades of research modelling quantum systems in classical computers has alluded the scientific community \autocite{boixo_characterizing_2016}. The development of near-term physical hardware \autocite{kelly_preview_2018}, \autocite{sete_functional_2016} has combined with a surge of interest to apply quantum computing to numerous fields in computation \autocite{chailloux_efficient_2017, farhi_quantum_2014, biamonte_quantum_2018, ciliberto_quantum_2018, cleve_quantum_1998}. Graph similarity and graph-isomorphism are long-standing difficulties in computer science. Many useful formulations of graph similarity exist such as compound matching in chemistry \autocite{han_topological_2015, hattori_development_2003, raymond_rascal:_2002}, machine vision \autocite{lades_distortion_1993} and web-search \autocite{brin_anatomy_1998}.  This problem has no tractable exact formulation for graphs with unknown node correspondence and as such approximate solutions are considered industry standard. More specifically we define whole-graph similarity
\begin{definition}{Whole Graph Similarity:}
Given two graphs $G_1(v_1,e_1)$ and $G_2(v_2,e_2)$ with possibly different numbers of vertices and edges, find an algorithm which returns a measure of similarity $S | S \in [0,1]$. Furthermore:
\begin{enumerate}
\item $S(G_1, G_1) = 1$
\item $S(G_1, G_2) = S(G_2, G_1)$
\end{enumerate}
\label{ref:similarity_proposal}
\end{definition}
\section*{Aim}
To investigate a quantum algorithmic approach to graph similarity and its applications this project will examine graph similarity by applying the recently proposed 'Quantum Approximate Optimisation Algorithm' (QAOA) \autocite{farhi_quantum_2014}. The QAOA can be formulated to reduce a combinatorial optimisation problem to a parameter search on around two variables. This project primarily aims to investigate if such an approach leads to any improvements in speed, accuracy or robustness over classical methods.\newline
A secondary objective is to extend the generated model of graph similarity into a real-world contextual use such as object tracking or common sub-graph matching for example. Currently it is unknown whether a quantum advantage will yield any benefits in speed, accuracy or robustness over classical counter-parts and hence makes a suitable topic for research.
\section*{Method}
There will be a large amount of theoretical work in the development and validation of a quantum or hybrid quantum/classical algorithms to tackle the problem of graph similarity. Testing will require a series of standardised sources as well as comparison results or implementations of classical algorithms. Due to the compute-heavy nature of simulating quantum systems it is likely the Magnus supercomputer at the Pawsey Super-computing Centre will need to be utilised. \textit{Python}, \textit{C/C++} and possibly \textit{Fortran} will be used to simulate various approaches and to create visualisations of resulting circuit designs.
\subsection*{Status}
This project does not follow from previous work commencing at the start of the 2018 academic year. This research is a collaboration between the \textit{Quantum dynamics and computation} research group and the department of \textit{Computer science and software engineering}.\newline
Currently, a general understanding of quantum computing and potential object detection methods are being investigated in addition to classical object-tracking frameworks with the aim of finding a suitable starting point to apply quantum methods. An investigation into state-of-the-art quantum simulations yields a number of possible methods and frameworks \autocite{smelyanskiy_qhipster:_2016, pednault_breaking_2017, boixo_simulation_2017, chen_64-qubit_2018, chen_classical_2018}. Preliminary-work on simulating the Quantum Approximate Optimisation Algorithm (QAOA) locally is underway.
\section*{Software and Hardware Requirements}
Costs are expected to be negligible as access to required software packages are openly available on-line or through the University of Western Australia. The majority of testing is to be run on personal machines. Use of the Pawsey Supercomputing Centre is available if needed based on an agreement with the University. 
\end{document}
